PIM-tree: A Skew-resistant Index for Processing-in-Memory

The performance of today's in-memory indexes is bottlenecked by the memory latency/bandwidth wall. Processing-in-memory (PIM) is an emerging approach that potentially mitigates this bottleneck, by enabling low-latency memory access whose aggregate memory bandwidth scales with the number of PIM nodes. There is an inherent tension, however, between minimizing inter-node communication and achieving load balance in PIM systems, in the presence of workload skew. This paper presents PIM-tree, an ordered index for PIM systems that achieves both low communication and high load balance, regardless of the degree of skew in the data and the queries. Our skew-resistant index is based on a novel division of labor between the multi-core host CPU and the PIM nodes, which leverages the strengths of each. We introduce push-pull search, which dynamically decides whether to push queries to a PIM-tree node (CPU -> PIM-node) or pull the node's keys back to the CPU (PIM-node -> CPU) based on workload skew. Combined with other PIM-friendly optimizations (shadow subtrees and chunked skip lists), our PIM-tree provides high-throughput, (guaranteed) low communication, and (guaranteed) high load balance, for batches of point queries, updates, and range scans. We implement the PIM-tree structure, in addition to prior proposed PIM indexes, on the latest PIM system from UPMEM, with 32 CPU cores and 2048 PIM nodes. On workloads with 500 million keys and batches of one million queries, the throughput using PIM-trees is up to 69.7x and 59.1x higher than the two best prior methods. As far as we know these are the first implementations of an ordered index on a real PIM system.

==> removed_sections.tex <==
\section{removed sections}

\subsection{Replicating the top part}

The first optimization is to replicate all nodes close to the root in
all PIM modules, so search operations can go through the top part with a single "push"
operation. This optimization is also explained in \cite{kang2021processing}.
We divide the tree horizontally into two parts, and refer the part closer
to the root as \defn{Layer 3(L3)}, the part closer to leaves as \defn{Layer 2(L2)}. All nodes
in L3 are replicated in all PIM modules, while all nodes in L2 are still distributed
as in \Cref{sec:pim_skip_list}.
% We need to modify PIM pointers to L3 nodes to
% identify which replica it points to: if a source node has a PIM pointer
% to L3 nodes, which can be a pointer between L3 nodes or an \UP pointer from L2 to L3,
% it points to the replica stored in the source node's host PIM module.

Replicating L3 takes more space. The size of L3 is decided by the tradeoff between space overhead
and communication reduction.
We set the height of L2 to be $\log P$, so $1/P$ keys reach L3, and the replicated L3 takes additional
$O(n)$ space.

Notice that the L3 maintained by each PIM module is a pure local data structure.
Multiple in-memory data structures can be used.
We implemented both a multi-threaded skip list and a multi-threaded (a,b)-tree.
% The skip list version is shown in \Cref{fig:replicated_upper_part} with all replicas of L3 nodes.

% Note that
% all pointers toward L3 nodes point to the replica in the source nodes' host PIM module,
% especially the \UP pointers of nodes in the top level of Layer 2 with keys $-\infty$ and $7$. All replicas of L3
% nodes are designed to have exactly the same local address, so address of any replica gives addresses to all repilcas.

% We implemented this data structure as a version on the real PIM system with $2560$ PIM modules.
% We set the possibility of the skip list to be $1/2$, so each key is expected be stored $2$ times.
% We call this number theoretical space amplification.
% Since $\log_2{2560} = 11.32$, we set the height of L2 to $12$, so only $1/4096$ nodes are in L3.
% After replicating L3, its theoretical space amplification is increased from $1/2048$ to $2560/2048$,
% which is $1.25$. The total theoretical space amplification is increased by $62.5\%$, to $3.25$.

\subsubsection{Push-Pull Search-replicate}
By replicating the L3, we can optimize the "push-pull" search: always do a "push" as
the first step. At the beginning of a query batch, we send queries in a round-robin way:
we divide queries evenly into $P$
sub-batches, and send each sub-batch to each PIM module for pointer chasing in L3. All PIM module
can do pointer chasing locally until reaching a node in L2, because each has
a complete L3 replica. This step is balanced, finishing in only $1$ communication round,
and causing constant communication for each query.
After that, we do the multi-step push-pull search in L2 as mentioned in
\Cref{sec:pim_skip_list}, until getting the result.

By Replicating L3, the communication and CPU work for each query is reduced
from $O(\log n)$ to $O(\log P)$. When the height of L2 is set to $12$, the CPU-PIM communication
rounds needed is reduced from \hongbo{todo} to $60$, according to our experiment.

\subsubsection{Scan-replicate}

Similar to push-pull search, we also divide scan queries into $P$ sub-batches and "push" them to the PIM modules
in a round-robin way, since all modules have the L3 replica.
Then the PIM modules will carry out pointer chasing until find the nodes in L2 involved in the scan queries.
In this way, we reduce the communication and CPU work for each query from $O(\log n)$ to $O(\log P)$,
where the range batch overlays an expected total of $O(n)$ existing keys.

\subsubsection{Insertion and Deletion-replicate}

If one insertion or deletion only influence nodes in L2, the process is kept the same
as in \Cref{sec:pim_skip_list}. However,
if it add or remove a node in L3, we'll need to apply this modification
to all L3 replicas. We do this by broadcast this operations to all PIM modules, then they
apply it to their local L3 copies separately.

Although all such modifications need to be broadcasted and executed
in all $P$ PIM modules, given that the height of L2 is $\log P$, only $1/P$ of all modifications make it to L3.
One solution can be built by replacing the search method in prior
work \cite{kang2021processing}.


\subsubsection{Insertion and Deletion-1}

In this section, we briefly introduce the basic idea and the main challenge in
insertion and deletion batches.
Details are introduced in section "Chunking", because they are very different
after that optimization.

% process
PIM-tree does insertions and deletions in two steps: (i) get the search trace
(ii) do modifications according to the search trace. The search trace is a list of pointers to nodes on the pointer-chasing path,
and can be recorded when doing "push-pull" search.
To insert a key, we insert new nodes to the right-hand side of the search trace.
Similarly, to remove a key, we remove the node with that key from
horizontal link lists.
In following "Insertion and Deletion" sections,
we'll assume that we've already get the search trace,
and focus on how to do modifications based on the search trace.

% challenge
The main challenge in the modification step is to solve both
conflicts and contention when
executing a batch of operations in parallel.
Without careful design, skewed workload can
easily cause conflicts: inserting multiple keys between two existed adjacent
keys causes parallel insertions to the right side of the same node,
and removing
consecutive keys causes parallel deletions on
consecutive nodes in horizontal link lists.

% solution
A classic approach to solve these conflicts is to use atomic operations, like compare-and-swap, when modifying pointers.
However, although this avoid conflicts that corrupting the data structure, it still causes contentions,
because these atomic operations are done to the same pointer.
%  One solution is to carefully
% controll the order of these atomic operations.
% A simpler way
% is to do these parallel pointer modifications is to do them on the CPU side:
Following our fundamental philosophy, we solve this by using the CPU side:
% We solve this by do these parallel pointer modifications is to do them on the CPU side:
we fetch all nodes on the search trace back to the CPU side, and derive the correct pointer by
shared memory algorithms, then apply all changes to the actual node in PIM modules at once. This ensure that all pointers
are modified only once.
% For example, we do parallel list contraction for deletions.
% As for the algorithm in basic PIM skip list, we do comparisons between search traces of different insertions in insertions, and
% we do parallel list contraction for deletions.

One possible solution of the "modification step" for basic PIM skip list is mentioned
in prior work \cite{kang2021processing}, while the "search" process is completely different.
Replacing their "search step" with our "push-pull search" gives the insertion/deletion algorithm for
the basic PIM tree.

% To insert a (key, value) pair into a skip list, we first do a random coin tossing to
% decide which level the insert will appear. In following sections, we call it \defn{height of an insert}.
% We then do a predecessor query on that key,
% to get the search trace from the root to the leaf of the predecessor key.
% The query is done by the "push-pull" method,
% and the path is stored in CPU cache. Finally, we generate and distribute nodes in the
% new horizontal chain, and insert these nodes to the right-hand side of the recorded
% predecessors by modifying their pointers. For deletions, similarly, we do a predecessor
% query to get the search trace, then remove the nodes with that key from the horizontal
% link list.

% The main challenge of \pimbalanced batch-parallel insertion and deletion is to solve
% the interfere between parallel operations in a \pimbalanced way. The adversary can
% easily cause these interferences: doing multiple insertions between two adjacent
% keys causes parallel insertions to the same places in horizontal link lists, and removing
% consecutive keys in the skip list causes parallel deletions on
% consecutive nodes in horizontal link lists.
% A classic way to solve these conflicts is to use atomic operations like compare-and-swap,
% however, these operations may cause imbalance because they may change the same pointer
% for multiple times, unless controlling the order of operations carefully. A simpler way
% is to do these parallel pointer modifications is to do them on the CPU side: fetch these
% nodes and their search traces back to CPU cache, derive the correct pointer by parallel
% shared memory algorithms, then apply all changes to the actual node in PIM modules at once.
% For inserts, we do comparisons between search traces of different insertions; for deletions,
% we do parallel list contraction.

% One method to do insertion and deletion while avoiding contention is mentioned
% in paper \hongbo{ref}. Though the way they do searches is quite different from
% ours, ..

